Online Simulation at Machine Level: A Systematic Review

The importance of simulation at machine level in industrial environments is steadily increasing especially in the design and commissioning phase. Using models during the operation phase together with the real machine or plant is referred to as online simulation. Online simulation is used for system monitoring, predictive analyses, decision support or online optimization and therefore has various advantages and a wide field of applications. This paper has the aim to characterize online simulation at machine level in industrial automation focusing on key technologies and common applications. Therefore, a set of 65 relevant publications, which are focusing on this subject, is found by database search, expert consultation, and snowballing. As key technological aspects, the used model types, interfaces and platforms, and the aspects of initialization and synchronization are further investigated. The results are interpreted and limitations, knowledge gaps and future prospects are discussed. The potential of online simulation at machine level especially arises due to the increasing availability of component and machine models from the design and commissioning phase, which can be reused for online simulation. Remaining challenges are identified concerning implementation, simulation platforms, model maintenance and especially in the field of synchronization.

==> abstract.tex <==
Due to model-based engineering methods and increasing use of virtualization techniques in Industry 4.0, a lot of simulation models concerning components and machines of industrial automation exist.
Using such behavioral models in parallel to the operation of the corresponding system is referred to as online simulation.

